A Crowd-enabled Solution for Privacy-Preserving and Personalized Safe Route Planning for Fixed or Flexible Destinations (Full Version)

Ensuring travelers' safety on roads has become a research challenge in recent years. We introduce a novel safe route planning problem and develop an efficient solution to ensure the travelers' safety on roads. Though few research attempts have been made in this regard, all of them assume that people share their sensitive travel experiences with a centralized entity for finding the safest routes, which is not ideal in practice for privacy reasons. Furthermore, existing works formulate safe route planning in ways that do not meet a traveler's need for safe travel on roads. Our approach finds the safest routes within a user-specified distance threshold based on the personalized travel experience of the knowledgeable crowd without involving any centralized computation. We develop a privacy-preserving model to quantify the travel experience of a user into personalized safety scores. Our algorithms for finding the safest route further enhance user privacy by minimizing the exposure of personalized safety scores with others. Our safe route planner can find the safest routes for individuals and groups by considering both a fixed and a set of flexible destination locations. Extensive experiments using real datasets show that our approach finds the safest route in seconds. Compared to the direct algorithm, our iterative algorithm requires 47% less exposure of personalized safety scores.

==> safepath/algos/rowscan.tex <==
% fetch-safety-scores($N'$)\;
% create priority queue $Q$\;
% $storeSh \gets \emptyset$, $storeS \gets \emptyset$\;
% $Q \gets Q$ $\cap$ create-route($s$)\;
% \While{$Q$ is not empty}{
%     $R \gets $remove-safest($Q$)\;
%     $u \gets $last-node$(R)$\;
%     \lIf{$u = d$}{ \Return{R} }
    
%     % update-store($store, R$)\;
%     % \eIf {$store$ contains $u$}{
%     %     $shortestR \gets get(store, v)$\;
%     %     \lIf{$L(R)<L(shortestR)$}{$store \gets store$ $\cap$ $(u,R)$}
%     % }{
%     %     $store \gets store$ $\cap$ $(u,R)$\;    
%     % }
%     $shortestR \gets get(storeSh, v)$\;
%     \If{$shortestR = \emptyset$ or $L(R) < L(shortestR)$}{
%         $storeSh \gets storeSh$ $\cup$ $(u,R)$\tcp*[l]{if $shortestR$ exists already then that must be safer that $R$}
%     }
%     $safestR \gets get(storeS, v)$\;
%     \lIf{$safestR = \emptyset$}{  $storeS \gets storeS$ $\cup$ $(u,R)$}
    
%     \For{$v \in neighbor(u)$}{
%         \lIf{$v = s $ || $R$ contains $v$}{$continue$}
%         \If{$L(R)+length(e_{uv})+euclidian$-$dist(v,d)>D$}{
%             $continue$\tcp*[l]{prune 1}
%         }
        
%         $shortestR \gets get(storeSh, v)$\;
%         \If {$L(shortestR)  \leq  L(R)+length(e_{uv})$}{
%             $continue$\tcp*[l]{prune 2}
%         }
%         $safestR \gets get(storeS, v)$\;
%         \If {$L(safestR)  \leq  L(R)+length(e_{uv})$}{
%             $continue$\tcp*[l]{prune 3 for memory efficiency}
%         } 
        
%         $newR \gets$ create-route$(r,v)$\; 
%         $Q \gets Q$ $\cap$ $newR$\;
%     }
% }

% $N^\prime, A_q \gets$ compute\_query\_area$(s, d, \delta, N)$\;
% $G_q, M_q \gets$ retrieve\_query\_group$(A_q)$\;
% $SS_q \gets$ compute\_SS$(G_q, M_q, A_q)$\;
% $N^{\prime\prime} \gets$ refine\_query\_area$(s, d, \delta, N^\prime, SS_q)$\;
% $SR \gets$ compute\_safest\_route$(s, d, \delta, N^{\prime\prime}, SS_q)$\;
% \Return $SR$\;
$supercells \gets \{\}$\;
$assigned[1\cdots x_c][1\cdots y_c] \gets \text{False}$\;
\For{$i=1$ to $x_c$}{
    \For{$j=1$ to $y_c$}{
        \lIf{$assigned[i][j]$ or $blank[i][j]$}{$continue$}
        $\Psi_{ij} \gets pSS(i,j)$\;
        $k \gets j+1$\;
        \While{$k \leq y_c$ and $\Psi_{ij} = pSS(i,k)$ and $\text{not }assigned[i][j]$}{
            $k \gets k+1$\;
        }
        $h \gets k-j$\;

        $w \gets 1$\;
        \For{$p=i+1$ to $x_c$}{
            $okay\gets \text{True}$\;
            \For{$q=j$ to $j+h$}{
                \If{$\Psi_{ij} \neq pSS(p,q)$ or $assigned[p][q]$}{
                    $okay \gets \text{False}$\;
                    $break$\;
                }
            }
            \lIf{$\text{not }okay$}{$break$}
            $w \gets w + 1$\;
        }
        $assigned[i\cdots i+w][j\cdots j+h]$\;
        $sc \gets$ create\_supercell($i,j,w,h$)\;
        $supercells \gets supercells \cup \{sc\}$\;
    }
}
\Return $supercells$\;

